Graph-Based Generative Representation Learning of Semantically and Behaviorally Augmented Floorplans

Floorplans are commonly used to represent the layout of buildings. In computer aided-design (CAD) floorplans are usually represented in the form of hierarchical graph structures. Research works towards computational techniques that facilitate the design process, such as automated analysis and optimization, often use simple floorplan representations that ignore the semantics of the space and do not take into account usage related analytics. We present a floorplan embedding technique that uses an attributed graph to represent the geometric information as well as design semantics and behavioral features of the inhabitants as node and edge attributes. A Long Short-Term Memory (LSTM) Variational Autoencoder (VAE) architecture is proposed and trained to embed attributed graphs as vectors in a continuous space. A user study is conducted to evaluate the coupling of similar floorplans retrieved from the embedding space with respect to a given input (e.g., design layout). The qualitative, quantitative and user-study evaluations show that our embedding framework produces meaningful and accurate vector representations for floorplans. In addition, our proposed model is a generative model. We studied and showcased its effectiveness for generating new floorplans. We also release the dataset that we have constructed and which, for each floorplan, includes the design semantics attributes as well as simulation generated human behavioral features for further study in the community.

==> tex/applications.tex <==
\subsection{TEMPORARY RESULTS}
% \begin{table*}[]
% \centering
% \begin{tabular}{|c|c|l|l|}
% \hline
% \multicolumn{1}{|l|}{}                & \textbf{Walk Length} & \textbf{N1\%, N2\%, N3\%, N4\%, N5\% = Weighted Average} &  \\ \hline
% \multirow{3}{*}{\textbf{Random Walk 2}} & \textbf{3}           & 0.12, 0.24, 0.23, 0.20, 0.18 = 40                   &  \\ \cline{2-4} 
%                                       & \textbf{5}           & 0.13, 0.27, 0.23, 0.18, 0.16 = 42                   &  \\ \cline{2-4} 
%                                       & \textbf{8}           & 0.14, 0.24, 0.22, 0.20, 0.18 = 42                   &  \\ \hline
% \multirow{3}{*}{\textbf{Random Walk 1}}     & \textbf{3}           &  0.13, 0.27, 0.22, 0.18, 0.17 = 0.41                                                   &  \\ \cline{2-4} 
%                                       & \textbf{5}           &  0.14, 0.26, 0.22, 0.18, 0.16 = 41                                                 &  \\ \cline{2-4} 
%                                       & \textbf{8}           & 0.09, 0.27, 0.23, 0.20, 0.18 = 0.39                                                    &  \\ \hline
% \end{tabular}
% \caption{Two different version of random walks for converting graphs to sequences, The results are the percentage of proxy graphs in first five nearest neighbours.(proxy graphs are result of running random walks multiple times and they are not seen in training data.) \todo{Create a section to describe the experiment, how the experiment is conducted, how the graph is generated, what are the metrics? How the random and BFS/DFS walks are different? We can run an evaluation to validate for inductivity. Our embedding fundamentally don't see walks before, therefore recall is not very high? Supplement the data set with proxy graphs.} \todo{How the 2 types of walks are generated? What are different experiments we are conducting? Number of walks? Etc.}}
% \end{table*}

% \usepackage{multirow}
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{|l|l|l|l|l|}
\hline
                                        & \textbf{Walk Length}        & \textbf{Proxy Seen In Training or Not} & \textbf{Rank of Graph by itself{[}1, 2, 3, 4, 5{]}(\%)} & \textbf{Rank of Proxy{[}1, 2, 3, 4, 5{]}(\%)} \\ \hline
\multirow{6}{*}{\textbf{Random Walk 1}} & \multirow{2}{*}{\textbf{3}} & \textbf{Y}                                                &  {[}99.9, 0.1, 0, 0, 0{]} & {[}0.1, 49, 2, 1, 1{]}                                                \\ \cline{3-5} 
                                        &                             & \textbf{N}                                                & {[}100, 0, 0, 0, 0{]}                                                        & {[}0, 40, 1, 1, 0.7{]}                                                \\ \cline{2-5} 
                                        & \multirow{2}{*}{\textbf{5}} & \textbf{Y}                                                & {[}100, 0, 0, 0, 0{]}                                                        & {[}0, 75, 4, 2, 1.6{]}                                                 \\ \cline{3-5} 
                                        &                             & \textbf{N}                                                &{[}100, 0, 0, 0, 0{]}                                                         &  {[}0, 41, 1, 1, 0.9{]}                                         \\ \cline{2-5} 
                                        & \multirow{2}{*}{\textbf{7}} & \textbf{Y}                                                & {[}100, 0, 0, 0, 0{]}                                   & {[}0, 57, 2, 1, 1{]}                       \\ \cline{3-5} 
                                        &                             & \textbf{N}                                                &{[}47, 18, 11, 9, 5{]}                                                          &{[}52, 74, 1, 0.5, 0.4{]}                                                  \\ \hline
\multirow{6}{*}{\textbf{Random Walk 2}} & \multirow{2}{*}{\textbf{3}} & \textbf{Y}                                                &   {[}100, 0, 0, 0, 0{]}                                                      &  {[}0.        , 83.5, 3.2, 1.9, 1.32{]}                                                \\ \cline{3-5} 
                                        &                             & \textbf{N}                                                & {[}99.2, 0.7, 0.        , 0.        , 0.        {]}                                                        &   {[}0.7, 54, 2.8, 1.8, 1.2{]}                                               \\ \cline{2-5} 
                                        & \multirow{2}{*}{\textbf{5}} & \textbf{Y}                                                & {[}100, 0, 0, 0, 0{]}                                                         &  {[}1, 44, 2 , 1, 1.1{]}                                                \\ \cline{3-5} 
                                        &                             & \textbf{N}                                                &   {[}100, 0, 0, 0, 0{]}                                                      &  {[}2, 47, 2.54, 1.69, 1.17 {]}                                                \\ \cline{2-5} 
                                        & \multirow{2}{*}{\textbf{7}} & \textbf{Y}                                                &   {[}83, 16, 0, 0, 0{]}                                                      &  {[}16, 16, 0, 0, 0{]}                                                \\ \cline{3-5} 
                                        &                             & \textbf{N}                                                & {[}100, 0, 0, 0, 0{]}                                                        &   {[}0.03, 27, 1, 1, 1{]}                                               \\ \hline
\end{tabular}
\caption{Two different version of random walks with different walk lengths are used for converting graphs to sequences. For each walk length the random walks run 10 times to generate sequences and 1 time for creating a proxy graphs. Then  We tested the models in two states whether proxy graphs are seen in training or not(Proxy Seen In Training or Not). The next column shows the rank percentage of query graph by itself within 5 nearest neighbours. The last column shows rank percentage of proxy graphs within five nearest neighbours. In a good model we should have as more as possible the graphs by theirself in first rank and more proxy graphs in nearest ranks. {\color{red} Progress May 15, model rank: Random Walk 1 walk length 5, Random Walk 2 walk length 5}}
\end{table*}

\subsection{Pairwise Similarity between Floorplans}
{\color{red} TODO: Major changes, it is similar to SIMAUD}

In this use case we demonstrate a pairwise comparison between input floorplan and its second nearest neighbour from the embedding space. Underline graphs of both floorplans are compared using a popular graph similarity distance metric, Graph Edit Distance (GED)~\cite{bunke1983distance}. The edit distance between $G1$ and $G2$, GED(G1, G2), is the count of edit operations that transform $G1$ into $G2$, where the edit operations on a graph $G$ can be an insertion or deletion of an edge or node. All edit operations have the same constant cost which is $1$. If two graphs are identical, their GED is $0$.

First, we retrieved a semantically similar design (second nearest neighbour) from the embedding space for the given input floorplan such that they have similar structural attributes but significantly different behavioral attributes, Figure~\ref{fig:application_similarity_static}. The GDP value is reported as $0$, showcasing that the graphs are similar in their design semantics. Average exit flow values and color-coded density heatmaps are also shown for both floorplans. Input floorplan yielded comparatively lower exit flow than its nearest neighbour found from the embedding.

In next scenario, we retrieved a behaviorally similar floorplan (second nearest neighbour) from the embedding space for the given floorplan such that they have similar behavioral attributes but significantly different design semantics. A GDP value of $10$ is reported from the graphs comparison, showcasing the two graphs are design semantically different. However, their corresponding floorplans yielded similar exit flow values. A GDP graph transformation as well as density heatmaps are shown, Figure~\ref{fig:application_similarity_dynamic}. 


\begin{figure}[H]
    \centering
    
    \begin{subfigure}[t]{0.9\linewidth}
    \begin{tabular}{c}
        \includegraphics[width=1.0\linewidth]{images/applications/case1_1_v2.pdf}
    \end{tabular}
    \caption{Two floorplans which are structurally similar (Graph Edit Distance (GED) = $0$) but have different crowd behavioral attributes.}
    \label{fig:application_similarity_static}
    \end{subfigure}
    
    \par\bigskip % force a bit of vertical whitespace
    
    \begin{subfigure}[t]{0.9\linewidth}
    \begin{tabular}{c}
        \includegraphics[width=1.0\linewidth]{images/applications/case1_2_v4.pdf}
    \end{tabular}
    \caption{Two floorplans which are behaviorally similar (having similar average exit flows) but design semantically different (Graph Edit Distance (GED) = $10$).}
    \label{fig:application_similarity_dynamic}
    \end{subfigure}
    
    \caption{Pairwise similarity comparison between input floorplan and queried nearest neighbour from the embedding space.}
    \label{fig:application_similarity}
\end{figure}



\subsection{Behavioral and Geometrically-powered Floorplans Retrieval}

{\color{red} TODO: Rewriting}

In this use case we demonstrate the potential of using our embedding approach to retrieve similar and related floorplans. We trained three models with the architecture described. The difference between these models is the considered features. First model is trained only with design semantic features, second only with behavioral features and the third with all of the features.

First, we trained the models over houseExpo dataset (Fig.~\ref{fig:case11}). The top row is the baseline and the only considered feature is node degree. All the neighbours have same structure with same node degree but different design semantic features. The middle row showcases an example for the model which considered only design semantic features. This embedding setting contains a $12$ dimensional design semantic vector, $11$ for room types and $1$ for room dimensions. Given an input floorplan, a set of $5$ nearest neighbors from the embedding space are retrieved. For an embedding space to be meaningful and valid, a queried graph (input floorplan) should have itself as the first nearest neighbor during a retrieval, and therefore, in the figure, the first neighbor is same as the queried floorplan itself. The first 4 nearest neighbours have almost same structure (same node types with different sizes). The last nearest neighbour also has same structure with one extra node. But still the majority of its sequences are similar to queried graph. The bottom row showcases an example of floorplans retrieval from a collectively trained model with both design semantic and behavioral features. In this case, the features dimension for each node is 21. The top 5 nearest neighbours for the same input floorplan are retrieved from the embedding. Since in this case all of the features are considered, the neighbours must follow similar structure, similar design semantic and also similar behavioral pattern. The behavioral performance of the floorplans are visualized as color-coded crowd trajectories in the images by room type color.

To show performance of our model over more complicated datasets, the model is trained one time with design semantic and another time with all features over our synthesized indoor dataset. For both cases the top 5 nearest neighbours are retrieved and depicted in Fig. \ref{fig:case22}.  Fig. \ref{fig:case33} depicts the top 5 nearest neighbours from the model trained over our urban dataset only with design semantic features.


% Fig. \ref{fig:tsne1} shows a t-Distributed Stochastic Neighbor Embedding (t-SNE) 3D visualization of 3000 random embedding vectors. As it is clear in embedding space we have some explicit clusters which must have similar properties. Three clusters are marked and two random floorplans from one of the marked clusters are shown. As expected, they have similar structure and design semantics.


\subsection{Generation of a Composite Floorplan}

{\color{red} It is not complete}

Embedding spaces have commonly been used to make predictions and retrieving similar objects given some input criterion or an object. In this use case we demonstrate that our embedding methodology can also be used to generate a compound floorplan with collective features given multiple floorplans with a set of completely or partially different features. Figure~\ref{fig:application_generation} showcases one such example. Two floorplans with $2$ and $3$ different room types respectively, are given as input to our autoencoder, and the first nearest neighbour is a composite floorplan consist of $5$ different room types. It not just contains all the features from input floorplans but also maintains a significant proportion of their geometric symmetries.

\begin{figure*}[tbp]
    \centering
    \includegraphics[width=0.8\textwidth]{images/applications/application_generation_v3.pdf}
    \caption{Generation of a single floorplan with combined features from an embedding space given two floorplans with different set of features as input. Nodes of underline graph for each floorplan are color-coded based on room types.}
    \label{fig:application_generation}
\end{figure*}

% %\begin{figure}[htp]
%  \centering
%  \includegraphics[width=8cm]{images/tsne_1.png}
%  \caption{3D TSNE plot of the 3000 embedding vectors that are selected randomly. As image shows, there are some distinct clusters in embedding space. These clusters show the performance of proposed model to capture hidden correlation between floorplans. For example two images are selected randomly from one of the marked clusters and both have similar structure and semantic design. \textcolor{blue}{MK: This image has a lot of potential, but currently is not communicating anything at all. Please think carefully about what message you want to communicate in this image} }
%  \label{fig:tsne1}
% \end{figure}

\begin{comment}
\begin{table}[htp]
\centering
\begin{tabular}{|l|c|c|c|}
\hline
\textit{\textbf{Ranks/Models}}          & \textbf{Model#1} & \textbf{Model#2} & \textbf{Model#3} \\ \hline
{First rank(query graph itself)} & 100\%                          & 100\%                   & 100\%                 \\ \hline
{Second rank(proxy graph)}       & 86\%                           & 83\%                    & 85\%                  \\ \hline
{Third rank(proxy graph)}        & 13\%                           & 13\%                    & 14\%                  \\ \hline
{Fourth rank(proxy graph)}       & 1\%                            & 3\%                     & 1\%                   \\ \hline
{Fifth rank(proxy graph)}        & 0                              & 2\%                     & 0                     \\ \hline
\end{tabular}
\caption{This table shows the percentage of the floorplans that have them-self as first nearest neighbours and the rank percentage of their proxy graphs.}
\label{tbl:percentt}
\end{table}
\end{comment}

% \vspace{-30pt}

\begin{figure*}
    \centering
    \begin{tabular}{cc}
        \includegraphics[width=0.99\textwidth]{images/experiments/jjk_with_crowd_traces_v2.pdf}
    \end{tabular}
    \caption{The top 5 nearest neighbours from the embedding space for three different models trained on HouseExpo dataset. The top row shows baseline graphs with their respective degrees. In the second row, neighbors are retrieved from the model trained with design semantic features. Third row shows neighbors which are retrieved from a model jointly trained with design semantic and human behavioral features.}
    \label{fig:case11}
\end{figure*}


\begin{figure*}
    \centering
    \begin{tabular}{c}
        \includegraphics[width=0.99\textwidth]{images/experiments/jjk2.pdf}
    \end{tabular}
    \caption{The top 5 nearest neighbours from the embedding space for two different models trained on synthesized indoor dataset. Top: neighbors which are retrieved from the model trained with design semantic features. Bottom: neighbors which are retrieved from a model jointly trained with design semantic and human behavioral features.}
    \label{fig:case22}
\end{figure*}

% % \vspace{-0.2cm}
% \begin{figure*}
%     \centering
%     \begin{tabular}{c}
%         \includegraphics[width=0.99\textwidth]{images/experiments/jjk3.pdf}
%     \end{tabular}
%     \caption{The top 5 nearest neighbours from the embedding space for the model trained on synthesized urban dataset. Neighbors are retrieved from the model trained with design semantic features.
%     }
%     \label{fig:case33}
% \end{figure*}

\begin{figure}
	\centering
	\includegraphics[width=\linewidth, height=5.5cm]{images/expert_study/experts-preferences_v3.pdf} \\	
	
	\caption{\label{figure:experts-pref} The green portion of the bars show the average rating of experts' identification of similarity between input floorplan and the retrieved neighbors from the embedding space. }
\end{figure}

==> tex/case-study.tex <==
% In this section, we evaluate the proposed model's result. We consider two cases to show the performance. First, we consider only the design semantic features and train a model. Second, we consider all the design semantic and human behavioral features and train a model. For both cases, we find the top 5 nearest floorplans in embedding space. A meaningful embedding space should lead to a case that each graph has its own as first nearest neighbor.
% As another metric, we generate one proxy graph for each floorplan. Proxy graphs are the result of running random walk one more time that makes different sequence for each floorplan. These proxy graphs are not involved in training. We feed them to the trained model and add their representative vectors to embedding space. Then we find the top 10 nearest neighbors for each floorplan. Having these proxy graphs in higher ranks shows the validity of embedding space. In addition for each case examples are provided and discussed. More details are provided in following sub-sections.

% \textcolor{blue}{MK: We have no images showing the different kinds of features we compute. Can we have a sequence of images showing: (a) raw layout, (b) annotated with design features, (c) annotated with human behavior features. If some of these features need to be reported as numbers -- then show as tables. }

% \textcolor{blue}{MK: Are these floorplans the most complex floorplans we can show in the dataset ? Nothing more complex than this ? }

% \subsection{Embedding With Design Semantic Features}
% % In this part we only consider semantic features of floor-plans. Then we embed them and evaluate the result. For evaluation we find the top 5 nearest neighbours of all floor-plans which two of them is shown in Fig. \ref{fig:res1}.
% In this study, we only consider the $12$ dimentional design semantic features. Eleven for room type and one for room dimension. Then random walk generates the sequences for each floorplan as training semples. The model has the same architecture and properties as described and the model is trained for 50 epochs.
% % , the \ref{} shows the loss values during training.

% % \begin{figure}[htp]
% %     \centering
% %     \includegraphics[width=8cm]{images/loss_case_1.png}
% %     \caption{Loos value during training. It is close to 0.}
% %     \label{fig:loss1}
% % \end{figure}


% For each floorplan the 5 top nearest neighbours are found and we calculate the rank of query floorplan between these neighbours. As mentioned in a valid embedding space, each floorplan must have itself as first nearest neighbour. We get $100\%$ for this case. As explained for each graph we have a proxy graph that is the result of another run of random walk. These proxy graphs are not seen in training. After training these proxy graphs are feed to model and the result vectors are added to embedding space. Since proxy graphs are another presentation for each floorplan, having them as close as to second rank shows the validity of embedding space. Therefor, we find the 10 top nearest neighbours and calculate the proxy graphs rank for each floorplan. The reason for top 10 nearest neighbours is to make sure we see them between neighbours. The results are shown in table \ref{table:res1} . The proxy graphs have second rank for $86\%$ of floorplans, $13\%$ in third rank and only $1\%$ in fourth rank. The reason that all of the proxy graphs are not seen in second rank is because our graphs are unidirectional and we allow having loop in random walk. The randomness in random walk could lead to sequences that is back and fourth between only two nodes or a repeated subsequence because of loop. In both cases the generated sequences are not presenting the graph properly. This situation also has dependency to node degrees in the graphs since next node in random walk is selected based on weighted probability of nodes degree. This can be addressed by running random walk more than one time for each node or avoiding loops, both in training and test time. 

% \begin{table}[htp]
% \centering
% \begin{tabular}{|c|c|}
% \hline
% \textbf{Ranks} & \textbf{Percentage} \\ \hline
% First rank(query graph itself)     & 100                 \\ \hline
% second ranks(proxy graph)   & 86                  \\ \hline
% Third rank(proxy graph)     & 13                  \\ \hline
% Fourth rank(proxy graph)    & 1                   \\ \hline
% Fifth rank(proxy graph)     & 0                   \\ \hline
% \end{tabular}
% \caption{Fist rank shows the percentage of floorplans that have their own as first neighbour. Other ranks show the percentage of floorplans that have proxy graphs in second, third, fourth and fifth rank. }
% \label{table:res1}
% \end{table}

% Fig. \ref{fig:case11} illustrates the top 5 nearest neighbours for two floorplans. For both of them, the query graph by itself is in first rank. 
% First query floorplan is a rare design and second one is a popular one and we have more similar samples in dataset. For first query, the second and third nearest neighbours have same structure, the hallway in the middle and two bedrooms, one kitchen and one bathroom around it. Though, they have different design semantic features as annotated in the image. For these three floorplans, random walk generates almost similar sequences with different features, for example with start from bathroom in all of them we have a closed set of possibilities. Fourth neighbour has close structure only with missing the kitchen node. We have only one sample with this structure in dataset and its corresponding sequences are a subset of query graph sequences. The last neighbour almost has same structure but the middle node is different. Its corresponding sequences have a node in difference and that is the reason it is ranked in fifth position. Fifth neighbour is not a rare design and we have some similar designs in dataset, the similarity of design semantic features leads to have it as first different neighbour.

% Fig. \ref{fig:tsne1} shows the TSNE 3D visualization of 3000 random embedding vectors. As it is clear in embedding space we have some explicit clusters which must have similar properties. Three clusters are marked and two random floorplans from one of the marked clusters are shown. As expected they have similar structure and design semantics. 



% % In this part we only consider semantic features of the floorplans, embed them into graphs and then trained our model. We find the top-5 nearest neighbours for all floorplans. We then quantify the performance of our model by calculating the percentage of nearest neighbours. For evaluation purposes, two queried graphs and their top-5 neighbours are presented in Figure~\ref{fig:case1}. 

% \begin{figure*}
%     \centering
%     \begin{tabular}{c}
%         \includegraphics[width=18cm,height=6cm]{images/case1_res.png}
%     \end{tabular}
%     \caption{In this image top 5 nearest neighbours of two floorplans are shown. First query is a rare design and the second one is a popular one. In both cases the query graph by itself has the first rank. In first query the second and third neighbours have similar structure with different design semantic features. Fourth neighbour is similar structurally and semantically with missing only one node. Fifth neighbours has similar structure with different semantic attributes. For second query all of them have same structure and similar design semantic features. Their ranks is based on difference in their semantic attributes.(Light Red=Hallway, Light Blue=Bedroom, Light Green=Bathroom, Light Yellow=Kitchen, Light Purple=Living room, Orange= Lobby, Dark Blue=Room}
%     \label{fig:case11}
% \end{figure*}

% % \begin{figure*}
% % \centering 
% % \setlength{\tabcolsep}{2pt}
% % \begin{tabular}{c c c c c c}
    
% %     \includegraphics[width=0.15\linewidth]{images/1_q1.png} &
% %     \includegraphics[width=0.15\linewidth]{images/1_q1_1.png} &
% %     \includegraphics[width=0.15\linewidth]{images/1_q1_2.png} &
% %     \includegraphics[width=0.15\linewidth]{images/1_q1_3.png} &
% %     \includegraphics[width=0.15\linewidth]{images/1_q1_4.png} &
% %     \includegraphics[width=0.15\linewidth]{images/1_q1_5.png} \\
    
% %     Query & First NN & Second NN & Third NN & Forth NN & Fifth NN \\
    
    
% %     \includegraphics[width=0.15\linewidth]{images/1_q2.png} &
% %     \includegraphics[width=0.15\linewidth]{images/1_q2_1.png} &
% %     \includegraphics[width=0.15\linewidth]{images/1_q2_2.png} &
% %     \includegraphics[width=0.15\linewidth]{images/1_q2_3.png} &
% %     \includegraphics[width=0.15\linewidth]{images/1_q2_4.png} &
% %     \includegraphics[width=0.15\linewidth]{images/1_q2_5.png} \\
    
% %     Query & First NN & Second NN & Third NN & Forth NN & Fifth NN \\
    
% % \end{tabular}

% % \caption{Case study1, top 5 nearest neighbours only with design semantci features. Each row shows the NNs for one floorplan. In both cases the first NN is the floorplan by itself. More explanantion \textcolor{blue}{MK: Its not sufficient just showing nearest neigbhors. We need to have some nice discussion and insights into why they are similar to each other, and why this is not immediately obvious} }
% % \label{fig:case2}
% % \end{figure*}

% % We run random walk for each graph two times and have two set of sequences for each floorplan. It is so we can consider the second sequences as proxy graphs. The proxy sequences do not participated in training and only used for evaluation. After training is done, proxy sequences must generate an embedding vector close to the original sequence. \usman{so we pass them from encoder and add them to the embedding space and calculate their rank as second nearest neighbours since always the graph by itself is the first rank (not clear)}. Table~\ref{table:casetbl1} shows percentage results from nearest neighbours.

% % Fig. illustrates the embedding space. The dimensional of the embedding vectors are deducted to 2 by TSNE. Two explicit cluster is selected and two floorplans out of that is shown.

% \begin{figure}[htp]
%     \centering
%     \includegraphics[width=8cm]{images/tsne_1.png}
%     \caption{3D TSNE plot of the 3000 embedding vectors that are selected randomly. As image shows, there are some distinct clusters in embedding space. These clusters show the performance of proposed model to capture hidden correlation between floorplans. For example two images are selected randomly from one of the marked clusters and both have similar structure and semantic design. \textcolor{blue}{MK: This image has a lot of potential, but currently is not communicating anything at all. Please think carefully about what message you want to communicate in this image} }
%     \label{fig:tsne1}
% \end{figure}


% % \begin{table*}[]
% % \centering
% % \scalebox{0.9}{
% % \begin{tabular}{|c|c|c|c|l|l|l|l|}
% % \hline
% % \textbf{ID} & \textbf{Features}                                               & \textbf{Query}                                             & \textbf{1st}                                               & \multicolumn{1}{c|}{\textbf{2nd}} & \multicolumn{1}{c|}{\textbf{3rd}} & \multicolumn{1}{c|}{\textbf{4rd}} & \multicolumn{1}{c|}{\textbf{5th}} \\ \hline
% % \textbf{0}  & \textbf{\begin{tabular}[c]{@{}c@{}}Type\\ Footage\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Bedroom\\ 11.5\end{tabular}     & \begin{tabular}[c]{@{}c@{}}Bedroom\\ 11.5\end{tabular}     & \multicolumn{1}{c|}{Bedroom}      & Bedroom                           & Bedroom                           & Bedroom                           \\ \hline
% % \textbf{1}  & \textbf{\begin{tabular}[c]{@{}c@{}}Type\\ Footage\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Bathroom\\ 8.42\end{tabular}    & \begin{tabular}[c]{@{}c@{}}Bathroom\\ 8.42\end{tabular}    & \multicolumn{1}{c|}{}             &                                   &                                   &                                   \\ \hline
% % \textbf{2}  & \textbf{\begin{tabular}[c]{@{}c@{}}Type\\ Footage\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Kitchen\\ 8.4\end{tabular}      & \begin{tabular}[c]{@{}c@{}}Kitchen\\ 8.4\end{tabular}      &                                   &                                   &                                   &                                   \\ \hline
% % \textbf{3}  & \textbf{\begin{tabular}[c]{@{}c@{}}Type\\ Footage\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Bedroom\\ 9.83\end{tabular}     & \begin{tabular}[c]{@{}c@{}}Bedroom\\ 9.83\end{tabular}     &                                   &                                   &                                   &                                   \\ \hline
% % \textbf{4}  & \textbf{\begin{tabular}[c]{@{}c@{}}Type\\ Footage\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Living room\\ 8.10\end{tabular} & \begin{tabular}[c]{@{}c@{}}Living room\\ 8.10\end{tabular} &                                   &                                   &                                   &                                   \\ \hline
% % \end{tabular}}
% % \end{table*}



% \subsection{Embedding With All Features}
% In this study we consider both design semantic and crowd behavioral features in graphs nodes. We do the same procedure like first study, first random walk and then embedding. The model is same as described model and it is trained for 50 epochs.

% The same evaluation is done for this study and table \ref{table:res2} shows the percentage for top 5 nearest neighbour. In this case again each floorplan has itself as first nearest neighbour. But the percentage of proxy graphs are changed. Since the dimension of feature vectors are increased there is possibility that there are some floorplan are more close to query graph.

% Fig. \ref{fig:case2} illustrate the top 5 nearest neighbours for same two floorplan in case one. As you see still the qurt floorplan by itself is in first rank but the others orders are changed. \todo{explain more}

% \begin{table}[H]
% \centering
% \begin{tabular}{|c|c|}
% \hline
% \textbf{Ranks} & \textbf{Percentage} \\ \hline
% First rank(query graph itself)     & 100                 \\ \hline
% second ranks(proxy graph)   & 81                  \\ \hline
% Third rank(proxy graph)     & 13                  \\ \hline
% Fourth rank(proxy graph)    & 3                   \\ \hline
% Fifth rank(proxy graph)     & 2                   \\ \hline
% \end{tabular}
% \caption{Fist rank shows the percentage of floorplans that have their own as first neighbour. Other ranks show the percentage of floorplans that have proxy graphs in second, third, fourth and fifth rank. }
% \label{table:res2}
% \end{table}

% % and embed them into graphs and then trained our model. For evaluation purposes, we query the same graphs as in first part and reported their top-5 nearest neighbours (Figure~\ref{fig:case2}). Results show that this time nearest neighbours are different because of embedding crowd behavioral features in the graphs. \usman{need to discuss more details. It is very trivial to show that we change the feature space and we are getting different neighbours. Does not really sound very scientific or something cool}



% % \usman{For quantifying, we repeat same strategy as case study1. For this case, we find top 5 nearest neighbours for all floor-plans and for all of them first nearest neighbour is the floorplans by itself. Same experiment with proxy graphs is done for this case study (not very clear)}. Table~\ref{table:casetbl2} shows percentage results from nearest neighbours.

% % \begin{table}[htb]
% % \centering
% % \begin{tabular}{|l|l|}
% % \hline
% % Ranks         & Percentage \\ \hline
% % Rank First NN(floorplan itself)   &    100        \\ \hline
% % Rank three NN(proxy floor-plan) &         81   \\ \hline
% % % Rank four NN  &            \\ \hline
% % % Rank five NN  &            \\ \hline
% % \end{tabular}
% % \caption{\usman{caption? Every table needs to have proper caption}}
% % \label{table:casetbl2}
% % \end{table}


% % \usman{Fig. illustrate the embedding space for this case, two explicit clusters are selected and two floorplans out of that cluster is shown (which figure you are referring to? Not very clear)}.

% % \subsection{Discussion}
% % We find also mutual NN and they are moreless same.

==> tex/expriments.tex <==
\begin{figure}
	\centering
	\includegraphics[width=\linewidth, height=5.5cm]{images/expert_study/experts-preferences_v3.pdf} \\	
	
	\caption{\label{figure:experts-pref} The green portion of the bars show the average rating of experts' identification of similarity between input floorplan and the retrieved neighbors from the embedding space. }
\end{figure}


% \todo{Vahid need to add details here...}
In this section we are showing the performance of our proposed model and importance of considered features with a set of experiments.
% Since our datasets are unlabeled \textcolor{red}{???}, a user study is conducted to verify the results.

In the first experiment, we are training three models over houseExpo dataset (Fig.~\ref{fig:case11}). The first model is the baseline and the only considered feature is node degree. 
% \Fig. \ref{fig:case11}. 
Then top 5 neighbours are retrieved and as the first row shows, all the neighbours have same structure with same node degree but different design semantic features. In second model, design semantic features are considered and as the second row shows first 4 nearest neighbours have almost same structure(same node types with different sizes). The last nearest neighbour also has same structure with one extra node. But still the majority of its sequences are similar to query graph. In third model all features are considered and the top 5 neighbours are shown in last row. As this row shows the nearest neighbours are arranged in a way to capture both design semantic and human behavioral features. The agents traces are visualized in the images by room type color.

To show performance of our model over complicated datasets, the model is trained one time with design semantic and another time with all features over our synthesized indoor dataset. For both cases the top 5 nearest neighbours are retrieved and depicted in Fig. \ref{fig:case22}.  Fig. \ref{fig:case33} depicts the top 5 nearest neighbours over our urban dataset only with design semantic features. For verification of these neighbours, the below user study is conducted.

\begin{figure*}
    \centering
    \begin{tabular}{cc}
        \includegraphics[width=0.99\textwidth]{images/experiments/jjk_with_crowd_traces_v2.pdf}
    \end{tabular}
    \caption{The top 5 nearest neighbours from the embedding space for three different models trained on HouseExpo dataset. The top row shows baseline graphs with their respective degrees. In the second row, neighbors are retrieved from the model trained with design semantic features. Third row shows neighbors which are retrieved from a model jointly trained with design semantic and human behavioral features.}
    \label{fig:case11}
\end{figure*}


\begin{figure*}
    \centering
    \begin{tabular}{c}
        \includegraphics[width=0.99\textwidth]{images/experiments/jjk2.pdf}
    \end{tabular}
    \caption{The top 5 nearest neighbours from the embedding space for two different models trained on synthesized indoor dataset. Top: neighbors which are retrieved from the model trained with design semantic features. Bottom: neighbors which are retrieved from a model jointly trained with design semantic and human behavioral features.}
    \label{fig:case22}
\end{figure*}

% \vspace{-0.2cm}
\begin{figure*}
    \centering
    \begin{tabular}{c}
        \includegraphics[width=0.99\textwidth]{images/experiments/jjk3.pdf}
    \end{tabular}
    \caption{The top 5 nearest neighbours from the embedding space for the model trained on synthesized urban dataset. Neighbors are retrieved from the model trained with design semantic features.
    }
    \label{fig:case33}
\end{figure*}

% \textcolor{red}{DS: guys, this does not look like a city/urban environment. I suggest removing this example.}

==> tex/frame1imgpath.tex <==
https://drive.google.com/file/d/1htu0w5A10ncPfiwHOhZcDMF8y7PWF7Nq/view?usp=sharing



% https://app.diagrams.net/?title=TVCJ%202020%20of%20floorplan_embedding_framework_v1.drawio

==> tex/introduction.tex <==
%Floorplans provide a well-established mean to represent buildings. As such, they afford a wide range of design activities such as ideation, analysis, evaluation and communication. Computer-Aided Design (CAD) and Building Information Modeling (BIM) approaches support the creation of digital building models, from which floorplans can be extracted. Current approaches, however, do not support the systematic comparison of floorplan features derived from geometric and semantic properties as well as more advanced performance metrics, such as space utilization and occupant behavior generated via simulation.

%While research mostly developed in Computer Graphics proposed computational strategies to extract  geometric floorplan features by processing them as images~\cite{mace2010system,dosch1999reconstruction} or  graphs~\cite{sharma2016unified,sabri2017semantic}, these approaches ignore semantic information that describes the function of each space, as well as time-based analytics of human movement and activities. Because of this, architects and planners do not have digital means to analyze, compare, and sort through a large number of floorplans that have similar of different features.

%To address this issue, we propose \textit{floorplan embedding} -- ``latent'' representations of building layouts  using an attributed graph as intermediate representation which facilitate semantically meaningful comparisons that account for not only design and structural features, but also human behavior features. Specifically, a Long Short-Term Memory (LSTM)  \cite{hochreiter1997long} autoencoder \cite{hinton1994autoencoders} is trained to represent these graphs as vectors in a continuous space. These vector representations are then used to cluster and query floorplans with similar characteristics and attributes. Some of the advantages of presenting floorplans as vectors are: (a) compact representation, (b) efficient way to compare designs and fast retrievals, (c) scoring designs and providing feedback/recommendations, and (d) categorizing design according to our target features. In addition, since there is not any dataset augmented with mentioned features, we release a novel annotated floorplan dataset with semantics and human behavioral features generated from simulations.

%In architectural design, it is a common practice that whenever a new building design is to be made, architects and designers make use of existing and previously built building plans as a starting reference to get immediate feedback or recommendation regarding their design.  Such a practice helps in providing insights on how similar architectural requirements and specifications were addressed in the previous design layouts. And then a new design solution (building layout) is derived, compliance with reference design layouts, for the current architectural scenario. This retrieval or comparison is mostly based on floorplan structure, and the important factors like design semantic features and the semantics of how people actually inhabit the space gets ignored. Since humans are inhabitants of these spaces, their interacts need to be encoded for any operation like finding similarity between floorplans. For example, the average time for evacuation in a room or building is an important safely factor.  To look for similar design layouts, in most cases, is a manual process and can consume a significant amount of time. Also, there is no floorplan dataset annotated with crowd behavioral features. With a rapid progression towards digitalization, architectural blueprints (floorplans) are too cataloged in digital formats. The increase in such catalogs of digital floorplans of buildings raises the opportunity for automated computational techniques to search and query similar floorplans w.r.t. given design criterion and other operation like clustering, and has also served as motivation for this work. 

{\color{red} TODO: Improving it and add more text}

Floorplan representations support a set of fundamental activities in the architectural design process such as the ideation and development of new designs, their analysis and evaluation with respect to selected performance criteria, and the communication among stakeholders. While Computer-Aided Design (CAD) and Building Information Modeling (BIM) approaches support the creation of digital building models from which floorplans can be extracted, these methods do not support the systematic comparison of floorplan features derived from geometric and semantic properties as well as more advanced performance metrics, such as space utilization and occupant behavior generated via simulation.

Recent developments proposed techniques for extracting information from floorplans by processing them as graphs~\cite{sharma2016unified,sabri2017semantic} or as images~\cite{mace2010system,dosch1999reconstruction}. However, these approaches ignore low-level design details like information about the area of a given room in square feet~\cite{nauata2020house}. In addition, the features with respect to behavior of humans that have the main interactions with buildings are missing. 
% Meaningful comparison of floorplans needs to consider these features. But so far there was not any floorplan dataset annotated with semantic and crowd behavioral features.}

We propose a novel mechanism for floorplan embeddings that uses a Long Short-Term Memory (LSTM) Variational Autoencoder (VAE) with attributed graphs as intermediate representations that consider not only the design semantics and low-level structural characteristics but also crowd behavioral attributes of potential human-building interactions. An experiment is presented to showcase floorplan retrievals from the embeddings on two different datasets: (i) a preprocessed houseExpo dataset~\cite{li2019houseexpo}, (ii) a new synthesized dataset for complex indoor floorplans. Further details on the datasets are available in Section~\ref{subsec:dataset}. A pilot expert user-study is also conducted to validate floorplan retrievals from embedding spaces with respect to their similarity with input floorplans. In addition, VAE is a generative model that can be used to generate meaningful floorplans.

%To best of our knowledge, it is the first time that floorplans are represented with attributed graphs and augmented with crowd behavioral features, and also that deep autoencoder model is utilized for representing floorplans as vector. 

Our contributions can be summarized as follows: (i) representation of floorplans as attributed graphs, augmented with design semantic and crowd behavioral features generated by simulation (ii) an unsupervised deep-learning model to learn a meaningful vector representation of floorplans using  LSTM Variational Autoencoder (iii) creation of two new synthesized datasets for indoor and urban layouts augmented with design semantic and crowd behavioral attributes generated via crowd simulations. 
% The effectiveness of the proposed embedding approach is demonstrated by showcasing two case studies. In these case studies we are considering each feature class separately and all together and retrieve the similar floorplans. furthermore, the floorplans are clustered for each case studies and some samples are showcased.

% \vspace{-40pt}

==> tex/methodology.tex <==
{\color{blue}
Fig. \ref{} illustrates the proposed framework, comprising of two components. The first component converts floorplans into attributed graphs augmented with design semantic and human behavioral features generated by simulation. The second component embeds the attributed graphs in a continues space. The details are provided in following sections.
}


\subsection{Dataset}
\label{subsec:dataset}

{\color{blue}
We used the houseExpo dataset \cite{li2019houseexpo} that includes $35,000$ 2D floorplan layouts in JavaScript Object Notation (JSON) format. There are 25 component types in this dataset where some of them share similar semantic labels (e.g. toilet and bathroom or terrace and balcony). We reduce the types to 10 including unknown label \ref{tbl:roomtypes} by removing less common semantics based on reported statistical metrics in dataset (e.g. freight elevator) and considering an unique type for similar proposes components. %A sparse and inaccurate labeling provided for room segments in this dataset. Either there is not any label for some segments or two or more semantically different labels for one room is provided. 
Additionally, we remove from the set the floorplans with inaccurate or missing labels. At the end of the process, we obtain 8775 floorplan layouts. Figure~\ref{fig:rawf} shows an image of a raw floorplan compiled as image.
}

\begin{table}[hbt]
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Room types} & \begin{tabular}[c]{@{}c@{}}Bathroom\\ Office\\ Garage\\ Dining\_Room\\ Bedroom\\ Living\_Room\\ Kitchen\\ Hall\\ Hallway\\ Unknown\end{tabular} \\ \hline
\end{tabular}
\label{tbl:roomtypes}
\caption{Available room types in datasets.}
\end{table}



\subsection{Floorplans to Graphs and Feature Augmentation}

{\color{blue}

In this step, raw floorplans are represented as an attributed graph in which rooms compose nodes and edges are their connectivity if there is an immediate door between room pairs. For this conversion houseExpo samples are compiled as image and by image processing techniques room segments and their connectivity are recognized. The connection direction is recognized as a part of this process. We consider four directions East, West, North and South. Finding connection between two room segments is from the room with high degree to node with low degree since our graphs is not directed.

Floorplans structure like number of rooms and their connectivity is encoded in graph structure. However, capturing structure is necessary but not enough. So, we are augmenting graphs nodes with design semantic and human behavioral features and edges are with direction features shown in Table \ref{table:feat}.
Design semantic features include room type with 10 dimensional one-hot vector and square footage with one scalar value. Human behavioral features are generated by simulation and include metrics regarding evacuation time, traveled distance, flow rate and the number of successful/unsuccessful agents to exit from corresponding building. All features in this class are presented with a scalar value and total dimension is 9.
% In houseExpo dataset, design semantic features are extracted by image processing techniques. 
To generate these behavioral features the 2D floorplans are converted to 3D models loadable in a crowd simulator, SteerSuits \cite{singh2009open}.  The simulator automatically populates virtual agents in each room with the target to exit the floorplan and features are calculated.

At the end of this step, the floorplans are presented as an attributed graph $G=(V, E)$ in which $V$ denotes its vertex set (room segments) and $E \subseteq VxV$ denotes its edges (connectivity between room pairs). Each node $v$ has a constant dimensional feature vectors $F_{v}$. Moreover, each edge $e$ has a constant feature vectors $F-{e}$. The nodes feature vector dimension is 11 and edge feature vector dimension is 4.
}


\begin{table}[htb]
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Node\\ Features\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Feature \\ Classes\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Feature \\ Types\end{tabular}}                                                                                                                                                                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Feature\\ Dimension\end{tabular}}               \\ \cline{2-4} 
                                                                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Design \\ Semantic\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Square Footage\\ Room Type\end{tabular}}                                                                                                                                                                         & \textbf{\begin{tabular}[c]{@{}c@{}}1\\ 11\end{tabular}}                            \\ \cline{2-4} 
                                                                                  & \textbf{Behavioral}                                                 & \textbf{\begin{tabular}[c]{@{}c@{}}Not completed agents\\ Max evacuation time\\ Min evacuation time\\ Exit flow rate\\ Completed agents\\ Max traveled distance\\ Ave evacuation time\\ Avg traveled distance\\ Min traveled distance\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}1\\ 1\\ 1\\ 1\\ 1\\ 1\\ 1\\ 1\\ 1\end{tabular}} \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Edge\\ Features\end{tabular}}                  & \textbf{\begin{tabular}[c]{@{}c@{}}Design\\ Semantic\end{tabular}}  & \textbf{Direction}                                                                                                                                                                                                                                  & \textbf{4}                                                                         \\ \hline
\end{tabular}
\end{table}


\subsection{Floorplan Embedding}
{\color{blue} 
We convert floorplans to attributed graphs which both nodes and edges have feature. These graph are representing floorplan geometry as well as it design semantics and behavioral features. These graphs can be used directly for comparing floorplans. However, Graph analysis are expensive in term of computation and space cost. This challenge addressed by proposing efficient methods for graph analysis like \cite{kumar2016g} but still they are not efficient and these methods do not represent graphs with a vector. Another solution for addressing complexity of graph analysis is graph embedding. Graph embedding maps the graphs to a low dimensional space while their properties are preserved. Particularly we are looking for a mapping function to map graph G to a n-dimensional vector which graph properties are reserved and graphs with similar properties are close in this n-dimensional embedding space.Graph embedding can mainly divided to node embedding, edge embedding, hybrid embedding and whole-graph embedding   \cite{DBLP:journals/corr/abs-1709-07604}.
In this study, the aim is to embed whole floorplan(graph) and other types are not in our focus. There is possibility to use partial embedding like node embedding and use the average of the node embedding vectors as whole-graph representation. But since in partial embedding the whole graph structure is not captured, they do not lead to good performance \cite{taheri2018learning}. 

% \cite{niepert2016learning}
Some whole-graph embedding methods relying on efficient calculation of graph similarities in graph classification tasks \cite{shervashidze2011weisfeiler}. These methods are supervised and need labeled dataset. Since, none of our datasets are labeled we need an unsupervised method. Graph2Vec\cite{narayanan2017graph2vec} is an unsupervised method that by maximizing the likelihood of graph subtrees given graph embedding generates representations. Since this model uses subgraphs for finding representation, the graph global information is not captured and causes low performance. In \cite{taheri2018learning} for capturing the whole-graph structures, they converted a graph to a set of sequences and proposed a LSTM autoencoder to learn graph representations. This method suits unattributed graphs and nodes are embedded for generating nodes feature vectors prior training. In \cite{DBLP:journals/corr/BowmanVVDJB15} and \cite{wang2019topic} Variational autoenocder is used for text and sentence embedding and generation which in both inputs are sequences. It motivates us to adapt their model both for embedding and generating floorplans \ref{fig:method}.

Long Short Term Memory, 
}

% % The floorplans are presented with attributed graphs in which graph structure captures floorplan geometry and semantics features are augmented as node features.
% % and \cite{kumar2016g}

% Graph analysis are expensive in term of computation and space cost. Some methods are proposed for efficient analysis on graphs like \cite{kumar2016g}. Graph embedding is another way to solve this problem. Graph embedding maps the graphs to a  low-dimensional space while the graph properties are preserved. 
% % Different graph types (heterogeneous, attributed graphs and etc.)  and variation in their format and size open many challenges.
% Graph embedding can mainly divided to node embedding, edge embedding, hybrid embedding and whole-graph embedding   \cite{DBLP:journals/corr/abs-1709-07604}.

% %  \cite{DBLP:journals/corr/GoyalF17}\honglu{what is this?}

% In this study, the aim is to embed whole floorplan(graph) and other types are not in our focus. There is possibility to use partial embedding like node embedding and use the average of the node embedding vectors as whole-graph representation. But since in partial embedding the whole graph structure is not captured, they do not lead to good performance 
% % in related applications like graph clustering 
% \cite{taheri2018learning}. Particularly we are looking for a mapping function to map graph G to a n-dimensional vector which graph properties are reserved and graphs with similar properties are close in this n-dimensional embedding space.

% % \cite{niepert2016learning}
% Some whole-graph embedding methods relying on efficient calculation of graph similarities in graph classification tasks \cite{shervashidze2011weisfeiler}. These methods are supervised and need labeled dataset. Since, none of our datasets are labeled we need an unsupervised method. Graph2Vec\cite{narayanan2017graph2vec} is an unsupervised method that by maximizing the likelihood of graph subtrees given graph embedding generates representations. Since this model uses subgraphs for finding representation, the graph global information is not captured and causes low performance. In \cite{taheri2018learning} for capturing the whole-graph structures, they converted a graph to a set of sequences and proposed a LSTM autoencoder to learn graph representations. This method suits unattributed graphs and nodes are embedded for generating nodes feature vectors prior training. In \cite{DBLP:journals/corr/BowmanVVDJB15} and \cite{wang2019topic} Variational autoenocder is used for text and sentence embedding and generation which in both inputs are sequences. It motivates us to adapt their model both for embedding and generating floorplans \ref{fig:method}.



% % Different type of graphs, like heterogeneous or attributed graphs open new challenges since the inputs are varying in format and size. Graph embedding mainly can be divided to partial embedding(node or sub-graph embedding like graphlet) and whole graph embedding. 

% % in this paper our focus is on whole graph embedding and we are not dealing with techniques for node or sub-graph embedding. As experimented in \cite{} using node or sub-graph embedding for generating whole graph embedding reduce the performance since partial embedding can not capture whole graph precisely. They do a good job in capturing local structures.

% % Some research effort like GraphX \cite{gonzalez2014graphx}

% % expensive in term of computation and space cost. There is some research effort to propose efficient analytic on graphs e.x. .

% % Graph embedding is another track to solve this problem. Graph embedding converts the graphs to a  low dimensional space while the graph properties are preserved.  Different type of graphs, like heterogeneous or attributed graphs open new challenges since the inputs are varying in format and size. Graph embedding mainly can be divided to partial embedding(node or sub-graph embedding like graphlet) and whole graph embedding. in this paper our focus is on whole graph embedding and we are not dealing with techniques for node or sub-graph embedding. As experimented in \cite{} using node or sub-graph embedding for generating whole graph embedding reduce the performance since partial embedding can not capture whole graph precisely. They do a good job in capturing local structures.

% % In following we are providing some definitions and the details regarding our embedding methods is provided.


% % \subsection{Definitions}
% % The floorplans are presented as an intermediate attributed graphs $G=(V, E)$. $V$ denotes its vertices that are the room segments and $E \subseteq VxV$ denotes its edges that are potential doors between rooms. Each node has a constant dimensional feature vectors $F_{v}$ that are the considered node features. Our datasets are unlabeled and we do not have label for graphs(floorplans), however floorplans can be labeled or multi-labeled based on layout types like single-family houses, apartment buildings or design types like luxury and simple or based on saftly metrics.





\subsection{Graphs to Sequences}
{\color{blue}
We can convert graphs to sequences by methods including not limited to Random walk or Breadth First Search(BFS). In \cite{taheri2018learning} they used Random walk, BFS and shortest path between all pairs of nodes. The experiments show sequences generated by random walk lead to a better embedding performance.

Random walk is used in \cite{Perozzi_2014} for converting graphs to sequences. In this version we pick a node and then randomly we pick an edge to move to its neighbours. We repeat this procedure until we get a walk of some predefined length. In \cite{grover2016node2vec} the random walk is modified to have two parameters $Q$ and $P$. Parameter $Q$ is the probability of discovering the undiscovered parts of the graph and parameter $Q$ is the probability for returning to the previous node. In \cite{taheri2018learning} they modified the random walk with adding probability $1/D(N)$, where $D(N)$ is the degree of node $N$. In this walk we start from a node and the next node will be selected by its probability $1/D(N)$.

We used both walks with different walk length to figure out which walk and which walk length leads to better result for us. We call the random walk proposed in \cite{grover2016node2vec} 'Random Walk 1' and the one presented in \cite{taheri2018learning} as 'Random Walk 2'. Beside node sequences, the edge sequences captured and then both are used for training the model.

% In this paper we use two versions of random walk for converting our graphs to sequences. The first version(Random walk 1) is the proposed one in \cite{grover2016node2vec}. The second one(Random walk 2) is a modified version of the proposed one in \cite{taheri2018learning}. In \cite{taheri2018learning} they worked with large graphs and most probably with their proposed random walk they tried to move toward nodes with low visibility chance. However, we are working with small graphs and consequently we need shorter walk length and moving to high degree nodes is more valuable for us to capture the dominant structure of the graph. Therefore, we move to neighbour nodes $N_n = {N_1, N_2, ..., N_m}$ of the selected node $N$ with probability $D(N_j)/\sum^{m}_{i=1}D(N_i),$ $j=\{1,...,m\}$. Along with node sequences, the edge sequences will be captured and both are then used for training the model.

}



% Graphs can converted to sequences by methods like Random walk, First breath search and Shortest path. Since random walks lead to better performance, we used random walk for generating sequences \cite{taheri2018learning}. In a random walk we start from a given source node and the next node will be selected randomly with probability $1/D(N)$, where $D(N)$ is the degree of node $N$. This step will be repeated for a fixed length $L$. The random walk length is a hyper parameter and has dependency to graphs size distribution in datasets. These sequences are used both as input and poutput in training.
% After training the average embedding vector of a graph sequences are used as graph representation.

% Each graph is converted to a set of sequences and these sequences are feed to the model for training. Length of random walk is a hyper parameter and mostly depends to graph size distribution in dataset. Though, acoording to our experiments considering a set of length instead of one lead to better performance.


% \subsection{Model}
% In \cite{}, they propose a LSTM autoencoder for embedding unattributed graphs in which the average embedding vectors of sequences are considered as graph representation. Since their graphs are unattributed they apply Weisfeiler-Lehman (WL) over graphs to learn an emebdding for graph nodes and then the node embedded vectors are used as node values.  In addition in \cite{} varitional autoencoder is purposed as powerful generative model for sentence generation and learn embedding vector in sentence space. It motivates us to adapt their model to our problem both for embedding floorplans and generating floorplans which can address the lack of datasets in this area.

\subsection{Model}
{\color{blue}
In this paper we present a LSTM variational Auto-encoder model for embedding our attributed graphs Fig. \ref{fig:vae_model}. As explained we have attributes both in nodes and edges with different dimension. To handle this difference in dimensionality, we consider two parallel LSTM VAE, one for node sequences and one for corresponding sequences. In training phase both branch loss function is added up. 
}

{\color{red} TODO: Completing this part, maybe it will integrated somewhere else.}

\begin{figure*}
	\centering
	\includegraphics[width=15cm, height=5cm]{images/vae_imgs/model.png} \\
	\caption{\label{fig:vae_model} {\color{blue} The proposed model with two parallel LSTM VAE, one for node sequences and one for corresponding edge sequences. Each branch loss function is added up at the end in training.} {\color{green} Does this reflect the most recent developments ? We need to greatly improve this image. Perhaps Honglu can help}
}
\end{figure*}



% Two experiments are done for training. In one of them all features are converted to categorical features and categorical cross entropy is used as loss function. In second experiments, except room type which is categorical features, other features are normalized in [0 1] and directly are used for training. Second experiment gives slightly better accuracy.

% In order to train the propose model, first we are converting graphs to a set of node sequences that each node has a constant length feature vectors. The length or set of Random walk length are defined based on graph sizes distribution in each dataset. Then these sequences are padded to have same size in training time and used as input and output for the model.
% We try both presenting feature vector as categorical and scalar value in which in first case we had categorical cross entropy as loss function and in second one Mean square error. We get slightly better result with scalar features.

% \todo{missing Training details...}

% This section talks about the conversion of attributed graphs into continues latent vectors which encode both structure and semantics of the floorplans, as well as their crowd behavioral features. We use graph embedding approach to transform graph nodes, edges, and their features into a vector space (lower dimensional) while preventing any information loss. Graphs, however, are tricky to deal with because they can vary in terms of their scale, specificity, and subject~\cite{cai2017comprehensive, Goyal_2018}.

% There exist some approaches to perform graph embedding~\cite{grover2016node2vec, tang2015line, taheri2018learning, narayanan2017graph2vec}. However, they are only suitable for unattributed graphs and mostly capture just the graph structure. But in our case, the graphs are attributed. So in order to account for these attributes, we proposed an (Long Short Term Memory) LSTM autoencoder. Auto-encoders~\cite{hinton1994autoencoders} are trained to learn the full properties of the data and reconstruct their inputs. They generally have two parts: an encoder that maps the input to an intermediate representation and a decoder that reconstructs the inputs from intermediate representation. The intermediate representations are latent vectors. LSTM is a recurrent neural network (RNN) for capturing long-distance dependencies in sequential data and also supports varying data lengths.

% We propose a LSTM autoencoder to learn embedding space in a way that keeps floorplans of similar structure, design semantic and crowd behavioral features, close to each another in the embedding space. Our proposed model is illustrated in Fig. \ref{fig:method}. We learn the function for mapping graph $G$ to vector $R$ in a d-dimensional space. In a floorplan (graph) $G=(V, E)$, $V$ denotes its vertex set (rooms) and $E$ $\subseteq$ $VxV$ denotes its edge set (potential doors between rooms). We have unlabeled graphs in our dataset. %In the current version, our dataset is unlabeled, but in the future, we can add a label to them based on some architectural factors. 
% Each node has a constant dimensional feature-vector $F_{V}$.

% Adjacency matrix is one of the ways to present graphs as input to algorithms. But since the graphs are varying in number of nodes and edges, presenting them as adjacency matrix opens new challenges. This is because the dimension of the adjacent matrix is different for different graphs. To address this, we convert graphs to multiple varying length sequences. This conversion is done by using Random Walk. In a random walk we start from a given source node and the next node will be selected randomly with probability $1/D(N)$, where $D(N)$ is the degree of node $N$. Each graph is converted to a set of sequences and these sequences are feed to the model for training. Then the average latent vectors of corresponding sequences to a graph are used as a representation vector for the graphs (Equation~\ref{eq:avg}).


% \begin{equation}
% 	\Phi(G) = \dfrac{1}{Nseq}\sum_{n=1}^{Nseq}RS_n
% 	\label{eq:avg}
% \end{equation}


% The $Nseq$ is the number of sequences and $RS$ is corresponding latent vector to each sequence.

% \subsection{Training}
% Some of malformed graphs are removed from the dataset. We use about $33000$ floorplans' graphs which are converted to a set of sequences.  
% % and final valid graphs are $x$. 
% We run random walks on the graphs to generate corresponding sequences. These sequences are feed into our model for training, both as input and output since the method is unsupervised. The loss function in our model is Mean Squared Error (MSE) (Equation 2).

% \begin{equation}
% 	loss(s) = \dfrac{1}{|s|} \sum_{i=1}^{|s|} \bar{Y} - Y
% \end{equation}

% Which $s$ is the given sequence and $|s|$ is the number of nodes in the sequence. $\bar{Y}$ is the reconstructed vector for a node and $Y$ is the true vector for that node. Loss function calculates the difference between reconstructed vector(output of decoder) and input sequences which each node has feature vectors $F_v$. In other words the encoder is trying to reconstruct the node features in the sequence.


% {\color{red}The below table shows the related accuracy, add training testing accuracy}


\begin{comment}
\begin{figure*}
    \centering
    \begin{tabular}{c}
        \includegraphics[width=14cm,height=6cm]{images/Model_2.png}
    \end{tabular}
    \caption{\textcolor{blue}{MK: I would consider integrating this into Figure 1 and making Figure 1 more complex} Proposed model, LSTM Autoiencoder. Right part shows the encoder that has 2 layer LSTM, first one has 84 and second one has 64 LSTM units. Left part shows decoder that has two LSTM layer, first one has 64 and the second one has 84 LSTM units(opposite to encoder).}
    \label{fig:modell}
\end{figure*}
\end{comment}

==> tex/new.tex <==
{\color{red} 

\begin{table*}[]
\centering
\begin{tabular}{|c|c|l|l|}
\hline
\multicolumn{1}{|l|}{}                & \textbf{Walk Length} & \textbf{N1\%, N2\%, N3\%, N4\%, N5\% = Aggregation} &  \\ \hline
\multirow{3}{*}{\textbf{Random Walk}} & \textbf{3}           & 0.12, 0.24, 0.23, 0.20, 0.18 = 40                   &  \\ \cline{2-4} 
                                      & \textbf{5}           & 0.13, 0.27, 0.23, 0.18, 0.16 = 42                   &  \\ \cline{2-4} 
                                      & \textbf{8}           & 0.14, 0.24, 0.22, 0.20, 0.18 = 42                   &  \\ \hline
\multirow{3}{*}{\textbf{BFS/DFS}}     & \textbf{3}           &  0.13, 0.27, 0.22, 0.18, 0.17 = 0.41                                                   &  \\ \cline{2-4} 
                                      & \textbf{5}           &  0.14, 0.26, 0.22, 0.18, 0.16 = 41                                                 &  \\ \cline{2-4} 
                                      & \textbf{8}           & 0.09, 0.27, 0.23, 0.20, 0.18 = 0.39                                                    &  \\ \hline
\end{tabular}
\caption{Two walking approaches for converting graphs to sequences, Random Walk and Node2Vec Walk. The results are the percentage of proxy graphs in first five nearest neighbours.(proxy graphs are result of running random walks multiple times and they are not seen in training data.) \todo{Create a section to describe the experiment, how the experiment is conducted, how the graph is generated, what are the metrics? How the random and BFS/DFS walks are different? We can run an evaluation to validate for inductivity. Our embedding fundamentally don't see walks before, therefore recall is not very high? Supplement the data set with proxy graphs.} \todo{How the 2 types of walks are generated? What are different experiments we are conducting? Number of walks? Etc.}}
\end{table*}

Summary:\\

In this paper we propose a novel graph embedding(whole graph embedding) method for floorplans embedding.\\

There are some works for floorplan representation but almost most of them 
12
 lost the important semantic features. In this paper we consider design semantic and behavioral features and represent floorplans by attributed graphs(attributes on nodes/edges) as intermediate representation. Node features are same as our last work but we are adding course of connection as edge features in the graphs.\\

There are many works for graph embedding in node level and a limited number of works for whole graph embedding. The average of embedded node vectors can be used as whole graph embedding but it is shown the aggregation of node embedding is not enough to captures graph structure. In addition, most of the whole graph embedding methods didn't consider node and edge features as a part of embedding and mostly focus on graph structure. In this paper we propose a whole graph embedding for attributed graphs. \\

The procedure:\\
1. Converting graphs to a bunch of sequences by random walk. In last work we had constant length for sequences and we run random walk for each node only one time. But in Deepwalk paper authors perform from 32 to 64 random walks from each node. They also show that good random walks have a length of about 40 steps. In this paper we are going to run random walks few time for each node and also with different length to find the best case. Also in Node2Vec paper they utilized a random walk which is the combination of BFS and DFS and we can use that as well. They explain that BFS capture local structure and DFS captures global graph structure and it can lead to a better graph representation.

2. Proposing a VAE for embedding graphs. In \cite{} they propose a VAE model for text generation. Already I implement their model and we can adapt it for our work and see we can also generate floorplan like original paper or not. There are two approaches for moving forward with this method, first we can run a node embedding methods over all graphs and get an embedding vector for their node and use those vectors for graph embedding. Second, we can add some information to nodes regarding their local aspects like node degree and then apply our model. Embedding nodes for each graphs will be tedious since we have a lot of graph and they are just small graphs. Most probably the node embedding methods won't converge to good result.
}

{\color{red}
In this paper we focus on floorplan representation and the method for embedding is proposed for this goal.
//
Novelties:
Presenting floorplans with attributed graph(nodes and edges)
Augmenting semantic and behavioral features
Proposing an VAE model for embedding floorplans
//
Experiments:
two walk types(random and the one in node2vec paper)
//
Comparison:
With SIMAUD paper


}

In this paper we propose a new graph embedding(whole graph embedding) and our application is floorplans embedding.

First, floorplans are represented as an attributed graphs(attributes on nodes and edges) and then we use VAE proposed in \cite{kingma2013autoencoding} for embedding.

steps:
presenting floorplans as graph(attributes on nodes and edges)

